Single-Shot Learning of Stable Dynamical Systems for Long-Horizon Manipulation Tasks

Mastering complex sequential tasks continues to pose a significant challenge in robotics. While there has been progress in learning long-horizon manipulation tasks, most existing approaches lack rigorous mathematical guarantees for ensuring reliable and successful execution. In this paper, we extend previous work on learning long-horizon tasks and stable policies, focusing on improving task success rates while reducing the amount of training data needed. Our approach introduces a novel method that (1) segments long-horizon demonstrations into discrete steps defined by waypoints and subgoals, and (2) learns globally stable dynamical system policies to guide the robot to each subgoal, even in the face of sensory noise and random disturbances. We validate our approach through both simulation and real-world experiments, demonstrating effective transfer from simulation to physical robotic platforms. Code is available at https://github.com/Alestaubin/stable-imitation-policy-with-waypoints

==> tex/extra.tex <==


\begin{figure}[t]
    \centering      
    \includegraphics[width=0.5\textwidth]{fig/HighLevel.png}
    \caption{Framework of the high-level controller.}
    \label{fig:high-level}
\end{figure}



\hc{}{}{Describe Fig.~\ref{fig:exp-robosuite-rollout}}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/2D-entire-traj-nn.png}            
        \caption{Behaviour Cloning}
        \label{fig:rollout-nn}
    \end{subfigure}
    \hfill \\
    
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/2D-entire-traj-snds.png}
        \caption{SNDS}
        \label{fig:rollout-snds}
    \end{subfigure}
    \caption{Policy rollouts with perturbations injected during the rollout}
    \label{fig:exp-robosuite-rollout}
\end{figure}

\hc{}{}{maybe 1 figure is enough? }




==> tex/table-deterministic.tex <==

\begin{table}[t]
\centering
\caption{Comparison of success $(1)$ and failure $(0)$ between the behavior cloning benchmark and our approach in a \textit{deterministic} environment across various tasks.}

\begin{tabular}{llccccc}
\toprule
\textbf{Task}& \textbf{Subgoal} & \textbf{BC} & \textbf{SNDS} & \textbf{BC + Seg.}& \textbf{Ours}\\ \midrule
Ketchup & 1       & $10.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$   & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$   & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\ \midrule
Square  & 1       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\ \midrule
Wine    & 1       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $60.0 \pm 0.0$  & $80.0 \pm 0.0$    & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\ \midrule
Bowl    & 1       & $10.0 \pm 0.0$  & $0.0 \pm 0.0$     & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\ \midrule
Cheese  & 1       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $100.0 \pm 0.0$  & $100.0 \pm 0.0$  & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$      & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\ \bottomrule
\end{tabular}
\label{table:deternimistic}
\end{table}

==> tex/table-noise-and-perturbation.tex <==

\begin{table}[t]
\centering
\caption{Success rate (\%) for behavior cloning benchmark and our work in a \textit{noisy} environment across various tasks.}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Task} & \textbf{Subgoal} & \textbf{BC + Seg.}& \textbf{Ours}\\ \midrule
Ketchup & 1       & $96.7  \pm 5.8$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $96.7  \pm 5.8$  & $\mathbf{100.0 \pm 0.0}$ \\ \midrule
Square  & 1       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $\mathbf{56.7 \pm 15.3}$        & $\mathbf{56.7 \pm 11.5}$ \\ \midrule
Wine    & 1       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $\mathbf{63.3 \pm 15.3}$        & $\mathbf{63.3 \pm 15.3}$ \\ \midrule
Bowl    & 1       & $90.0 \pm 17.3$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $83.3 \pm 20.8$        & $\mathbf{97.6 \pm 5.8}$ \\ \midrule
Cheese  & 1       & $80.0 \pm 26.5$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $100.0 \pm 0.0$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $100.0 \pm 0.0$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $80.0 \pm 26.5$        & $\mathbf{93.3 \pm 11.5}$ \\ \bottomrule

\end{tabular}
\label{table:noise-success-rates}
\end{table}



\begin{table}[t]
\centering
\caption{Success rate (\%) for behavior cloning benchmark and our work in a \textit{perturbed and Noisy} environment across various tasks.}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Task} & \textbf{Subgoal} & \textbf{BC + Seg.} & \textbf{Ours} \\ \midrule
Ketchup & 1       & $73.3  \pm 5.8 $  & $\mathbf{93.3  \pm 5.8}$ \\
        & 2       & $\mathbf{96.7  \pm 5.8}$   & $\mathbf{96.7  \pm 5.8}$ \\
        & 3       & $96.7  \pm 5.8$   & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $60.0  \pm 10.0$  & $\mathbf{80.0  \pm 0.0}$ \\ \midrule
Square  & 1       & $\mathbf{70.0 \pm 0.0}$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 2       & $66.7 \pm 5.8$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 3       & $90.0 \pm 17.3$         & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $53.3 \pm 11.5$         & $\mathbf{70.0 \pm 0.0}$ \\ \midrule
Wine    & 1       & $\mathbf{90.0 \pm 0.0}$         & $\mathbf{90.0 \pm 0.0}$ \\
        & 2       & $30.0 \pm 30.0$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 3       & $30.0 \pm 30.0$         & $\mathbf{80.0 \pm 17.3}$ \\
        & total   & $20.0 \pm 17.3$         & $\mathbf{50.0 \pm 10.0}$ \\ \midrule
Bowl    & 1       & $56.7 \pm 5.8$         & $\mathbf{93.3 \pm 11.5}$ \\
        & 2       & $90.0 \pm 10.0$         & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $93.3 \pm 11.5$         & $\mathbf{97.6 \pm 5.8}$ \\
        & total   & $46.7 \pm 15.3$         & $\mathbf{70.0 \pm 0.0}$ \\ \midrule
Cheese  & 1       & $33.3 \pm 32.1$        & $\mathbf{60.0 \pm 26.5}$ \\
        & 2       & $53.3 \pm 20.8$        & $\mathbf{60.0 \pm 0.0}$ \\
        & 3       & $90.0 \pm 17.3$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $16.7 \pm 11.5$        & $\mathbf{50.0 \pm 10.0}$ \\ \bottomrule
\end{tabular}
\label{table:noise-pert-success-rates}
\end{table}



==> tex/table-task.tex <==

\begin{table}[t]
\centering
\caption{Overview of the task demonstrations used.}
\begin{tabular}{@{}llrrr@{}}
\toprule
\textbf{Task}   & \textbf{Dataset} & \textbf{Demo \#}   & \textbf{Demo} & \textbf{Waypoints}\\ 
                &                  &                    & \textbf{length} & \textbf{Length }\\ \midrule
Ketchup & LIBERO-90       & 1 & 230 & 25 \\ \midrule
Square  & Robomimic       & 0 & 127 & 20 \\ \midrule
Wine    & LIBERO-Goal     & 4 & 158 & 24\\ \midrule
Bowl    & LIBERO-90       & 0 & 92 & 18\\ \midrule
Cheese  & LIBERO-Goal     & 1 & 92 & 14 \\ \bottomrule
\end{tabular}
\label{table:demos-and-waypoints}
\end{table}

==> tex/table.tex <==




\begin{table}[t]
\centering
\caption{Success rate (\%) for behavior cloning benchmark and our work in a \textit{noisy} environment across various tasks.}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Task} & \textbf{Subgoal} & \textbf{BC + Seg.}& \textbf{Ours}\\ \midrule
Ketchup & 1       & $96.7  \pm 5.8$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $96.7  \pm 5.8$  & $\mathbf{100.0 \pm 0.0}$ \\ \midrule
Square  & 1       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $\mathbf{56.7 \pm 15.3}$        & $\mathbf{56.7 \pm 11.5}$ \\ \midrule
Wine    & 1       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $\mathbf{63.3 \pm 15.3}$        & $\mathbf{63.3 \pm 15.3}$ \\ \midrule
Bowl    & 1       & $90.0 \pm 17.3$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $\mathbf{100.0 \pm 0.0}$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $83.3 \pm 20.8$        & $\mathbf{97.6 \pm 5.8}$ \\ \midrule
Cheese  & 1       & $80.0 \pm 26.5$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 2       & $100.0 \pm 0.0$        & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $100.0 \pm 0.0$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $80.0 \pm 26.5$        & $\mathbf{93.3 \pm 11.5}$ \\ \bottomrule

\end{tabular}
\label{table:noise-success-rates}
\end{table}


\begin{table}[t]
\centering
\caption{Success rate (\%) for behavior cloning benchmark and our work in a \textit{perturbed} environment across various tasks.}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Task} & \textbf{Subgoal} & \textbf{BC + Seg.} & \textbf{Ours} \\ \midrule
Ketchup & 1       & $73.3  \pm 5.8 $  & $\mathbf{86.7  \pm 5.8}$ \\
        & 2       & $70.0  \pm 10.0$  & $\mathbf{93.3  \pm 5.8}$ \\
        & 3       & $76.7  \pm 25.2$  & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $50.0  \pm 0.0 $  & $\mathbf{63.3  \pm 5.8}$ \\ \midrule
Square  & 1       & $\mathbf{70.0 \pm 0.0}$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 2       & $66.7 \pm 5.8$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 3       & $80.0 \pm 17.3$         & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $\mathbf{66.7 \pm 5.8}$         & $63.3 \pm 5.8$ \\ \midrule
Wine    & 1       & $\mathbf{86.7 \pm 5.8}$         & $\mathbf{86.7 \pm 5.8}$ \\
        & 2       & $36.7 \pm 25.2$         & $\mathbf{60.0 \pm 0.0}$ \\
        & 3       & $36.7 \pm 25.2$         & $\mathbf{73.3 \pm 23.1}$ \\
        & total   & $20.0 \pm 17.3$         & $\mathbf{40.0 \pm 10.0}$ \\ \midrule
Bowl    & 1       & $50.0 \pm 17.3$         & $\mathbf{97.6 \pm 5.8}$ \\
        & 2       & $83.3 \pm 5.8$         & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $86.7 \pm 5.8$         & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $26.7 \pm 15.3$         & $\mathbf{76.6 \pm 5.8}$ \\ \midrule
Cheese  & 1       & $30.0 \pm 26.5$        & $\mathbf{53.3 \pm 15.3}$ \\
        & 2       & $43.3 \pm 25.2$        & $\mathbf{56.7 \pm 5.8}$ \\
        & 3       & $90.0 \pm 17.3$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $13.3 \pm 11.5$        & $\mathbf{46.7 \pm 5.8}$ \\ \bottomrule
\end{tabular}
\label{table:pert-success-rates}
\end{table}
Note that, the Square task has a tight approach angle. 
We did not use a complex orientation planning algorithm, which is why the success rate is low. 
When the trajectory is perturbed, however, the approach angle changes and the success rate goes up.
\hc{}{if we are going to explain square, we need to explain the rest}{}

\begin{table}[t]
\centering
\caption{Success rate (\%) for behavior cloning benchmark and our work in a \textit{perturbed and Noisy} environment across various tasks.}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Task} & \textbf{Subgoal} & \textbf{BC + Seg.} & \textbf{Ours} \\ \midrule
Ketchup & 1       & $73.3  \pm 5.8 $  & $\mathbf{93.3  \pm 5.8}$ \\
        & 2       & $\mathbf{96.7  \pm 5.8}$   & $\mathbf{96.7  \pm 5.8}$ \\
        & 3       & $96.7  \pm 5.8$   & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $60.0  \pm 10.0$  & $\mathbf{80.0  \pm 0.0}$ \\ \midrule
Square  & 1       & $\mathbf{70.0 \pm 0.0}$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 2       & $66.7 \pm 5.8$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 3       & $90.0 \pm 17.3$         & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $53.3 \pm 11.5$         & $\mathbf{70.0 \pm 0.0}$ \\ \midrule
Wine    & 1       & $\mathbf{90.0 \pm 0.0}$         & $\mathbf{90.0 \pm 0.0}$ \\
        & 2       & $30.0 \pm 30.0$         & $\mathbf{70.0 \pm 0.0}$ \\
        & 3       & $30.0 \pm 30.0$         & $\mathbf{80.0 \pm 17.3}$ \\
        & total   & $20.0 \pm 17.3$         & $\mathbf{50.0 \pm 10.0}$ \\ \midrule
Bowl    & 1       & $56.7 \pm 5.8$         & $\mathbf{93.3 \pm 11.5}$ \\
        & 2       & $90.0 \pm 10.0$         & $\mathbf{100.0 \pm 0.0}$ \\
        & 3       & $93.3 \pm 11.5$         & $\mathbf{97.6 \pm 5.8}$ \\
        & total   & $46.7 \pm 15.3$         & $\mathbf{70.0 \pm 0.0}$ \\ \midrule
Cheese  & 1       & $33.3 \pm 32.1$        & $\mathbf{60.0 \pm 26.5}$ \\
        & 2       & $53.3 \pm 20.8$        & $\mathbf{60.0 \pm 0.0}$ \\
        & 3       & $90.0 \pm 17.3$        & $\mathbf{100.0 \pm 0.0}$ \\
        & total   & $16.7 \pm 11.5$        & $\mathbf{50.0 \pm 10.0}$ \\ \bottomrule
\end{tabular}
\label{table:noise-pert-success-rates}
\end{table}


\hc{}{}{
\begin{itemize}
    \item are those all from robosuite? any other dataset we need to cite?
    \item double check square/with pert. both are $56.7$ but different std 
\end{itemize}
}
\al{}{Square is from robomimic, I added the citation}
\al{}{Square with noise, both have mean 56.7, but dif stddev: avg(4,6,7) for bc, avg(5,5,7) for ours.}
\newcommand{\perfect}{\mathbf{100.0 \pm 0.0}}

\begin{table*}[t]
\centering
\caption{Success rate with and without noisy observations}
\begin{tabular}{|ll|rrrr|rrrr|}
\hline\hline
            &   & \multicolumn{4}{|c|}{\bf Without Observation Noise} & \multicolumn{4}{|c|}{\bf With Observation Noise} \\ 
\midrule
\textbf{Task}& \textbf{Subgoal} & \textbf{BC} & \textbf{SNDS} & \textbf{BC + Seg.}& \textbf{Ours} & \textbf{BC} & \textbf{SNDS} & \textbf{BC + Seg.}& \textbf{Ours}\\ 
\midrule
Ketchup & 1       & $nn.n \pm nn.n$  & $nn.n \pm nn.n$ & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $96.7 \pm 5.8$  & $\perfect$ \\
        & 2       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $\perfect$ & $\perfect$ \\
        & 3       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $\perfect$ & $\perfect$ \\
        & total   & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      &  $96.7 \pm 5.8$  & $\perfect$ \\
        \midrule
Square  & 1       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $\perfect$ & $\perfect$ \\
        & 2       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $\perfect$ & $\perfect$ \\
        & 3       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $\perfect$ & $\perfect$ \\
        & total   & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $nn.n \pm nn.n$  & $nn.n \pm nn.n$      & $56.7 \pm 15.3$  & $56.7 \pm 15.3$ \\
        \midrule
Wine    & 1       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $\perfect$ & $\perfect$ \\
        & 2       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $\perfect$ & $\perfect$ \\
        & 3       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $\perfect$ & $\perfect$ \\
        & total   & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $63.15 \pm 15.3$  & $63.15 \pm 15.3$ \\
        \midrule
Bowl    & 1       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $\perfect$ & $\perfect$ \\
        & 2       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $\perfect$ & $\perfect$ \\
        & 3       & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $\perfect$ & $\perfect$\\
        & total   & $- \pm -$  & $- \pm -$      & $\perfect$ & $\perfect$ & $- \pm -$  & $- \pm -$  & $83.3 \pm 20.8$  & $\mathbf{97.6 \pm 5.8}$ \\
\hline\hline
\end{tabular}
\label{table:success-rates}
\end{table*}

\begin{table*}[b]
\centering
\caption{Overview of the task demonstrations used.}
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Task} & \textbf{Dataset} & \textbf{Full Name} & \textbf{Demo \#} & \textbf{Demo length} & \textbf{Waypoints length }\\ \midrule
Ketchup & LIBERO-90       & put\_the\_ketchup\_in\_the\_top\_drawer\_of\_the\_cabinet\_demo & 1 & 230 & 25 \\ \midrule
Square  & Robomimic       & Square  & 0 & 127 & 20 \\ \midrule
Wine    & LIBERO-Goal     & put\_the\_wine\_bottle\_on\_the\_rack\_demo  & 4 & 158 & 24\\ \midrule
Bowl    & LIBERO-90       & put\_the\_white\_bowl\_on\_top\_of\_the\_cabinet\_demo & 0 & 92 & 18\\ \midrule
Cheese  & LIBERO-Goal     & put\_the\_cream\_cheese\_in\_the\_bowl\_demo  & 1 & 92 & 14 \\ \bottomrule
\end{tabular}
\label{table:tasks}
\end{table*}
